Reddit Rules and Rulers: Quantifying the Link Between Rules and Perceptions of Governance across Thousands of Communities

Rules are a critical component of the functioning of nearly every online community, yet it is challenging for community moderators to make data-driven decisions about what rules to set for their communities. The connection between a community's rules and how its membership feels about its governance is not well understood. In this work, we conduct the largest-to-date analysis of rules on Reddit, collecting a set of 67,545 unique rules across 5,225 communities which collectively account for more than 67% of all content on Reddit. More than just a point-in-time study, our work measures how communities change their rules over a 5+ year period. We develop a method to classify these rules using a taxonomy of 17 key attributes extended from previous work. We assess what types of rules are most prevalent, how rules are phrased, and how they vary across communities of different types. Using a dataset of communities' discussions about their governance, we are the first to identify the rules most strongly associated with positive community perceptions of governance: rules addressing who participates, how content is formatted and tagged, and rules about commercial activities. We conduct a longitudinal study to quantify the impact of adding new rules to communities, finding that after a rule is added, community perceptions of governance immediately improve, yet this effect diminishes after six months. Our results have important implications for platforms, moderators, and researchers. We make our classification model and rules datasets public to support future research on this topic.

==> covar_balance/balance_not_a_rule.tex <==
\begin{table}[H]
\centering
\label{tab:balance_not_a_rule}
\begin{tabular}{lccccc}
\toprule
Covariate & \makecell{Mean of Reference\\Population} & \makecell{Mean of Control\\Group (no rule)} & \makecell{Mean of Treated\\Group (has rule)} & SMD for Control & SMD for Treated \\
\midrule
Community Size & 1661.26 & 1761.95 & 1156.85 & 0.00 & -0.03 \\
Discussion & 0.11 & 0.11 & 0.12 & 0.00 & 0.00 \\
Hobby & 0.51 & 0.51 & 0.52 & -0.01 & 0.03 \\
Identity & 0.17 & 0.17 & 0.16 & 0.00 & 0.00 \\
Media & 0.14 & 0.14 & 0.13 & 0.00 & -0.01 \\
Memes & 0.05 & 0.05 & 0.05 & 0.00 & -0.01 \\
News & 0.02 & 0.03 & 0.02 & 0.01 & -0.06 \\
\bottomrule
\end{tabular}
\end{table}

